Putting the Squeeze on Array Programs: Loop Verification via Inductive Rank Reduction

Automatic verification of array manipulating programs is a challenging problem because it often amounts to the inference of in ductive quantified loop invariants which, in some cases, may not even be firstorder expressible. In this paper, we suggest a novel verification tech nique that is based on induction on userdefined rank of program states as an alternative to loopinvariants. Our technique, dubbed inductive rank reduction, works in two steps. Firstly, we simplify the verification problem and prove that the program is correct when the input state con tains an input array of length B or less, using the length of the array as the rank of the state. Secondly, we employ a squeezing function g which converts a program state sigma with an array of length > B to a state g(sigma) containing an array of length minus 1 or less. We prove that when g satisfies certain natural conditions then if the program violates its specification on sigma then it does so also on g(sigma). The correctness of the program on inputs with arrays of arbitrary lengths follows by induction. We make our technique automatic for array programs whose length of execution is proportional to the length of the input arrays by (i) perform ing the first step using symbolic execution, (ii) verifying the conditions required of g using Z3, and (iii) providing a heuristic procedure for syn thesizing g. We implemented our technique and applied it successfully to several interesting arraymanipulating programs, including a bidirec tional summation program whose loop invariant cannot be expressed in firstorder logic while its specification is quantifier free.

==> fig-exper-preds.tex <==
% !TEX root = vmcai2020.tex

\begin{table}[t]
\centering
\renewcommand\arraystretch{1.2}
\begin{tabular}{l@{~}|@{~}l}
\textbf{Program}   & \textbf{Predicates} \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\prog{strnchr(c) } & \prog{s[0]==c}, \prog{s[0]\!=c}, \prog{s[0]==0}, \prog{s[0]\!=0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
%%%%%%%%%%%%%%%%
\prog{strncmp} &
%%%%%%%%%%%%%%%%
\prog{s1[0]==s2[0]},
\prog{s1[0]\!=s2[0]},
\prog{s1[0]==0},
\prog{s2[0]==0},
\prog{s1[0]\!=0},
\prog{s2[0]\!=0}
%%%%%%%%%%%%%%%%
\\
%%%%%%%%%%%%%%%%%
\prog{max\_ind} &
%%%%%%%%%%%%%%%%%
\prog{s[0]<=s[1]},
\prog{s[0]<=s[2]},
\prog{s[0]<=s[n-2]},
\prog{s[0]<=s[n-1]},
\prog{s[1]<=s[2]},
%%%%%%%%%%%%%%%%%%%%%
\\              &
%%%%%%%%%%%%%%%%%%%%%
\prog{s[1]<=s[n-2]},
\prog{s[1]<=s[n-1]},
\prog{s[2]<=s[n-1]},
\prog{s[n-2]<=s[n-1]} 
%%%%%%%%%%%%%%%%%%%%%
\\ 
%%%%%%%%%%%%%%%%%
\prog{min\_ind} &
%%%%%%%%%%%%%%%%%
\prog{s[0]>=s[1]},
\prog{s[0]>=s[2]},
\prog{s[0]>=s[n-2]},
\prog{s[0]>=s[n-1]},
\prog{s[1]>=s[2]},
%%%%%%%%%%%%%%%%%
\\              &
%%%%%%%%%%%%%%%%%
\prog{s[1]>=s[n-2]},
\prog{s[1]>=s[n-1]},
\prog{s[2]>=s[n-1]},
\prog{s[n-2]>=s[n-1]} 
%%%%%%%%%%%%%%%%%%%%%
\\
%%%%%%%%%%%%%%%%%%
\prog{sum\_bidi} &
%%%%%%%%%%%%%%%%%%
\prog{i==0},
\prog{l==0},
\prog{r==0},
\prog{s[0]==0},
\prog{s[n-i]==0}
%%%%%%%%%%%%%%%%%%
\\
%%%%%%%%%%%%%%%%%%%
\prog{is\_sorted} &
%%%%%%%%%%%%%%%%%%%%%
\prog{s[n-3]<=s[n-2]},
\prog{s[n-3]<=s[n-1]},
\prog{s[n-2]<=s[n-1]}
%%%%%%%%%%%%%%%%%%%%%
\\
%%%%%%%%%%%%%%%%%%%
\prog{long\_pref} &
%%%%%%%%%%%%%%%%%%%
\prog{s[0]<=s[1]},
\prog{s[0]<=s[2]},
\prog{s[1]<=s[2]},
\prog{s[0]>s[1]},
%%%%%%%%%%%%%%%%%%%
\\                &
%%%%%%%%%%%%%%%%%%%
\prog{s[0]>s[2]},
\prog{s[1]>s[2]} 
%%%%%%%%%%%%%%%%%%%
%\\
\end{tabular}
\vspace{0mm}
\caption{User-supplied atom predicates used to synthesize $\sq$.}
\label{Ta:ExperPred}
\end{table}


==> fig-exper-ver-12col.tex <==
% !TEX root = vmcai2020.tex

%%%%%%%%%%%
%         %
% Table 2 %
%         %
%%%%%%%%%%%
\begin{table}[t]
\hspace{-4ex}\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r}
%%%%%%%%%%%%%%%%%
% MULTI COLUMNS %
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{1}{ c }{           } &
\multicolumn{4}{|c|}{\bf Phase 1} &
\multicolumn{4}{|c|}{\bf Phase 2} &
\multicolumn{4}{|c}{\bf Phase 3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
%%%%%%%%%%%%%%%%%%%%%%
\textbf{Program}     &
$|$\textbf{\scriptsize Pos.}$|$  &
   \textbf{\scriptsize  Time}     &
\textbf{\scriptsize $|$Neg.$|$} &
   \textbf{\scriptsize Time}     &
   \textbf{\scriptsize $|$Pos.$|$}  &
   \textbf{\scriptsize Time}     &
  $\textbf{\scriptsize $|$\textbf{Neg.}$|$}$ &
  $\textbf{\scriptsize Time}   $  & 
  \textbf{\scriptsize $|$Pos$|$ {}} &
   \textbf{\scriptsize Time}     &
  $\textbf{\scriptsize \textbf{$|$Neg.$|$}}$ &
  $\textbf{\scriptsize Time}$  
%$|$\textbf{\scriptsize Pos.}$|$  &
%   \textbf{\scriptsize Time}     &
%  $\textbf{\scriptsize Time}_{\tiny  | \textbf{Neg.} |}$ &
%$|$\textbf{\scriptsize Pos.}$|$  &
%   \textbf{\scriptsize Time}     &
%  $\textbf{\scriptsize Time}_{\tiny  | \textbf{Neg.} |}$
%%%%%%%%%%%%%%%%%%%%%%
\\ \hline
%%%%%%%%%%%%%%%%
\prog{strnchr} &
%%%%%%%%%%%%%%%%
1              & % Num phase 1 positives
$\epsilon$     & % Average time to test positive
9              & % Average num states to discriminate negative
$\epsilon$     & % Average time to test negative
1              & % Num phase 2 positives
0.94           & % Average time to test positive
$-$  & $-$          & % Average time to test negative
1              & % Num phase 3 positives
0.98           & % Average time to test positive
$-$ & 
$-$              % Average time to test negative
%%%%%%%%%%%%%%%%
\\
%  %%%%%%%%%%%%%%%%%
%  \prog{strrnchr} &
%  %%%%%%%%%%%%%%%%%
%  2               & % Num phase 1 positives
%  $\epsilon$      & % Average time to test positive
%  36              & % Average num states to discriminate negative
%  $\epsilon$      & % Average time to test negative
%                  & % Num phase 2 positives
%  6.37            & % Average time to test positive
%  4.09            & % Average time to test negative
%                  & % Num phase 3 positives
%  0               & % time to test positive
%                  & % time to test negative
%
% %%%%%%%%%%%%%%%%%
%  \\
%%%%%%%%%%%%%%%%
\prog{strncmp} &
%%%%%%%%%%%%%%%%
3              & % Num phase 1 positives
$\epsilon$     & % Average time to test positive
36             & % Average num states to discriminate negative
$\epsilon$     & % Average time to test negative
3              & % Num phase 2 positives
14.29          & % Average time to test positive
$-$ & $-$        & % Average time to test negative
3              & % Num phase 3 positives
2751           & % Average time to test positive
$-$ & 
$-$              % Average time to test negative
%%%%%%%%%%%%%%%%%
\\
%%%%%%%%%%%%%%%%%
\prog{max\_ind} &
%%%%%%%%%%%%%%%%%
11              & % Num phase 1 positives
$\epsilon$      & % Average time to test positive
3               & % Average num states to discriminate negative
$\epsilon$      & % Average time to test negative
2               & % Num phase 2 positives
0.78            & % Average time to test positive
1.08            & % Average time to test negative
1               & % Num phase 3 positives
31              & % Average time to test positive
0.41              % Average time to test negative

%%%%%%%%%%%%%%%%%
\\
%%%%%%%%%%%%%%%%%
\prog{min\_ind} &
%%%%%%%%%%%%%%%%%
11              & % Num phase 1 positives
$\epsilon$      & % Average time to test positive
7               & % Average num states to discriminate negative
$\epsilon$      & % Average time to test negative
2               & % Num phase 2 positives
0.91            & % Average time to test positive
1.19            & % Average time to test negative
1               & % Num phase 3 positives
16              & % Average time to test positive
0.43              % Average time to test negative
%%%%%%%%%%%%%%%%%
\\
%%%%%%%%%%%%%%%%%%
\prog{sum\_bidi} &
%%%%%%%%%%%%%%%%%%
12               & % Num phase 1 positives
$\epsilon$       & % Average time to test positive
1                & % Average num states to discriminate negative
0.05             & % Average time to test negative
1                & % Num phase 2 positives
0.56             & % Average time to test positive
0.69             & % Average time to test negative
1                & % Num phase 3 positives
16               & % Average time to test positive
$-$                % Average time to test negative

%%%%%%%%%%%%%%%%%%
\\
%%%%%%%%%%%%%%%%%%%
\prog{long\_pref} &
%%%%%%%%%%%%%%%%%%%
2                 & % Num phase 1 positives
$\epsilon$        & % Average time to test positive
74                & % Average num states to discriminate negative
$\epsilon$        & % Average time to test negative
1                 & % Num phase 2 positives
1.03              & % Average time to test positive
1.22              & % Average time to test negative
1                 & % Num phase 3 positives
0.89              & % time to test positive
$-$                 % time to test negative
%%%%%%%%%%%%%%%%%
\\
\end{tabular}
\caption{Experimental results. Time in seconds. $\epsilon \leq 10^{-4}$}
\label{Table_Experimental_results_statistics_data}
\end{table}

